MedCalc-Bench: Evaluating Large Language Models for Medical Calculations

As opposed to evaluating computation and logic-based reasoning, current benchmarks for evaluating large language models (LLMs) in medicine are primarily focused on question-answering involving domain knowledge and descriptive reasoning. While such qualitative capabilities are vital to medical diagnosis, in real-world scenarios, doctors frequently use clinical calculators that follow quantitative equations and rule-based reasoning paradigms for evidence-based decision support. To this end, we propose MedCalc-Bench, a first-of-its-kind dataset focused on evaluating the medical calculation capability of LLMs. MedCalc-Bench contains an evaluation set of over 1000 manually reviewed instances from 55 different medical calculation tasks. Each instance in MedCalc-Bench consists of a patient note, a question requesting to compute a specific medical value, a ground truth answer, and a step-by-step explanation showing how the answer is obtained. While our evaluation results show the potential of LLMs in this area, none of them are effective enough for clinical settings. Common issues include extracting the incorrect entities, not using the correct equation or rules for a calculation task, or incorrectly performing the arithmetic for the computation. We hope our study highlights the quantitative knowledge and reasoning gaps in LLMs within medical settings, encouraging future improvements of LLMs for various clinical calculation tasks.

==> tables/main_results.tex <==
\begin{table}[h!] \small
    \centering
    \caption{\textsc{MedCalc-Bench} accuracy of different systems. All numbers are in percentages.}
    \begin{tabular}{lc|cccc|ccc|c}
        \toprule
        \multirow{3}{*}{\bf Model} & \multirow{3}{*}{\bf Size} & \multicolumn{4}{c|}{\bf Equation} & \multicolumn{3}{c|}{\bf Rule-based} & \multirow{3}{*}{\bf Avg.} \\
        \cmidrule(lr){3-9}
         &  & Lab & Phy. & Date & Dos. & Risk & Sev. & Dia. & \\
        \midrule
        \multicolumn{10}{c}{\bf Zero-shot Direct Prompting} \\
        \midrule
PMC-LLaMA \cite{wu2024pmc} & 13B & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  \\
\textsc{MediTron} \cite{chen2023meditron} & 70B & \makecell{3.67\\\textcolor{gray}{\scriptsize$\pm$0.01}}  & \makecell{8.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{5.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{7.50\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{5.00\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{13.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{6.21\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Mistral \cite{jiang2023mistral} & 7B & \makecell{10.70\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{18.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{3.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{4.58\\\textcolor{gray}{\scriptsize$\pm$0.01}}  & \makecell{3.75\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{13.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{9.84\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Mixtral \cite{jiang2024mixtral} & 8x7B & \makecell{12.23\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{23.33\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{5.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{7.50\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{12.92\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{7.50\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{16.67\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \makecell{14.23\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 8B & \makecell{10.70\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{19.17\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{3.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{5.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{12.50\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{8.75\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{25.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{13.09\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 70B & \makecell{18.04\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{33.33\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{8.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{12.50\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \makecell{15.83\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{13.75\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{33.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{20.82\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
GPT-3.5 \cite{ouyang2022training} & N/A & \makecell{17.13\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{35.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{13.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{5.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{12.92\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{6.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{18.33\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \makecell{18.82\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
GPT-4 \cite{openai2023gpt4} & N/A & \makecell{14.37\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{34.58\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{38.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{14.58\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{20.00\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \makecell{20.82\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
        \midrule
        \multicolumn{10}{c}{\bf Zero-shot CoT Prompting} \\
        \midrule
PMC-LLaMA \cite{wu2024pmc} & 13B & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  \\
\textsc{MediTron} \cite{chen2023meditron} & 70B & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{3.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{3.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{0.38\\\textcolor{gray}{\scriptsize$\pm$0.00}}  \\
Mistral \cite{jiang2023mistral} & 7B & \makecell{10.09\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{14.58\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{1.67\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{9.58\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{7.50\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{25.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{10.79\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Mixtral \cite{jiang2024mixtral} & 8x7B & \makecell{22.63\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{40.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{6.67\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{17.50\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{11.25\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{21.25\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \makecell{22.35\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 8B & \makecell{16.51\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{25.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{1.67\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{7.50\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{11.25\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{13.75\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{26.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{16.43\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 70B & \makecell{33.94\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{66.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{25.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{20.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{18.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{16.25\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{36.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{35.53\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
GPT-3.5 \cite{ouyang2022training} & N/A & \makecell{20.49\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{45.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{11.67\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{17.50\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{13.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{10.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{31.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{23.69\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
GPT-4 \cite{openai2023gpt4} & N/A & \makecell{26.30\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{71.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{48.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{40.00\\\textcolor{gray}{\scriptsize$\pm$0.08}}  & \makecell{27.50\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{28.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{37.92\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
        \midrule
        \multicolumn{10}{c}{\bf One-shot CoT Prompting} \\
        \midrule
PMC-LLaMA \cite{wu2024pmc} & 13B & \makecell{5.20\\\textcolor{gray}{\scriptsize$\pm$0.01}}  & \makecell{10.42\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{8.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{2.50\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{7.08\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{1.25\\\textcolor{gray}{\scriptsize$\pm$0.01}}  & \makecell{11.67\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{6.97\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
\textsc{MediTron} \cite{chen2023meditron} & 70B & \makecell{22.94\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{39.58\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{31.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{20.42\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{31.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{26.27\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Mistral \cite{jiang2023mistral} & 7B & \makecell{11.01\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{30.42\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{6.67\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \makecell{16.25\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{6.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{18.33\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \makecell{16.05\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Mixtral \cite{jiang2024mixtral} & 8x7B & \makecell{28.13\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{50.83\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{8.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{22.50\\\textcolor{gray}{\scriptsize$\pm$0.07}}  & \makecell{21.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{8.75\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{33.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{29.23\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 8B & \makecell{34.86\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{35.42\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{3.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{2.50\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \makecell{20.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{11.25\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{41.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{27.13\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 70B & \makecell{41.59\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{56.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{30.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{22.50\\\textcolor{gray}{\scriptsize$\pm$0.07}}  & \makecell{27.50\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{27.50\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \makecell{45.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{39.45\\\textcolor{gray}{\scriptsize$\pm$0.02}}  \\
GPT-3.5 \cite{ouyang2022training} & N/A & \makecell{30.89\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{59.17\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{41.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{23.33\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{17.50\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \makecell{35.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{34.86\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
GPT-4 \cite{openai2023gpt4} & N/A & \makecell{51.68\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{77.50\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{46.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{37.50\\\textcolor{gray}{\scriptsize$\pm$0.08}}  & \makecell{33.75\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \makecell{27.50\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \makecell{53.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \makecell{50.91\\\textcolor{gray}{\scriptsize$\pm$0.02}}  \\
        \bottomrule
    \end{tabular}
    \label{tab:main_results}
\end{table}



==> tables/main_results_colored.tex <==

\begin{table}[h!] \small
    \centering
    \caption{\textsc{MedCalc-Bench} accuracy of different systems. All numbers are in percentages.\guangzhi{Choose one of them.}}
    \begin{tabular}{lccccc|ccc|c}
        \toprule
        \multirow{3}{*}{\bf Model} & \multirow{3}{*}{\bf Size} & \multicolumn{4}{c|}{\bf Equation} & \multicolumn{3}{c|}{\bf Rule-based} & \multirow{3}{*}{\bf Avg.} \\
        \cmidrule(lr){3-9}
         &  & Lab & Phy. & Date & Dos. & Risk & Sev. & Dia. & \\
        \midrule
        \multicolumn{10}{c}{\bf Zero-shot Direct Prompting} \\
        \midrule
PMC-LLaMA \cite{wu2024pmc} & 13B & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  \\
\textsc{MediTron} \cite{chen2023meditron} & 70B & \cellcolor{red!59.7!} \makecell{3.67\\\textcolor{gray}{\scriptsize$\pm$0.01}}  & \cellcolor{red!56.2!} \makecell{8.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!30.0!} \makecell{5.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!42.9!} \makecell{7.50\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!47.7!} \makecell{5.00\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!45.0!} \makecell{13.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!53.0!} \makecell{6.21\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Mistral \cite{jiang2023mistral} & 7B & \cellcolor{red!30.5!} \makecell{10.70\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!33.7!} \makecell{18.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!45.0!} \makecell{3.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!55.4!} \makecell{4.58\\\textcolor{gray}{\scriptsize$\pm$0.01}}  & \cellcolor{red!54.5!} \makecell{3.75\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!45.0!} \makecell{13.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!40.2!} \makecell{9.84\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Mixtral \cite{jiang2024mixtral} & 8x7B & \cellcolor{red!24.1!} \makecell{12.23\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!22.5!} \makecell{23.33\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!30.0!} \makecell{5.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!30.0!} \makecell{7.50\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!19.6!} \makecell{12.92\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!34.1!} \makecell{7.50\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!37.5!} \makecell{16.67\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \cellcolor{red!24.7!} \makecell{14.23\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 8B & \cellcolor{red!30.5!} \makecell{10.70\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!31.9!} \makecell{19.17\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!45.0!} \makecell{3.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!45.0!} \makecell{5.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!25.0!} \makecell{11.67\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!27.3!} \makecell{8.75\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!18.7!} \makecell{25.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{red!29.4!} \makecell{12.89\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 70B & \cellcolor{green!0.0!} \makecell{18.04\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!0.0!} \makecell{33.33\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!0.0!} \makecell{8.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{green!0.0!} \makecell{12.50\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \cellcolor{green!0.0!} \makecell{17.50\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!0.0!} \makecell{13.75\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{green!0.0!} \makecell{33.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!0.0!} \makecell{21.20\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
GPT-3.5 \cite{ouyang2022training} & N/A & \cellcolor{red!3.8!} \makecell{17.13\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!2.8!} \makecell{35.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!9.4!} \makecell{13.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!45.0!} \makecell{5.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!28.6!} \makecell{10.83\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!40.9!} \makecell{6.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!33.7!} \makecell{18.33\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \cellcolor{red!10.1!} \makecell{18.34\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
GPT-4 \cite{openai2023gpt4} & N/A & \cellcolor{red!15.2!} \makecell{14.37\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!2.1!} \makecell{34.58\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!56.3!} \makecell{38.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!6.8!} \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{red!5.4!} \makecell{16.25\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!6.8!} \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!30.0!} \makecell{20.00\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \cellcolor{green!0.0!} \makecell{21.20\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
        \midrule
        \multicolumn{10}{c}{\bf Zero-shot CoT Prompting} \\
        \midrule
PMC-LLaMA \cite{wu2024pmc} & 13B & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  \\
\textsc{MediTron} \cite{chen2023meditron} & 70B & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!45.0!} \makecell{3.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!67.5!} \makecell{3.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!73.6!} \makecell{0.38\\\textcolor{gray}{\scriptsize$\pm$0.00}}  \\
Mistral \cite{jiang2023mistral} & 7B & \cellcolor{red!33.0!} \makecell{10.09\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!42.2!} \makecell{14.58\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!60.0!} \makecell{1.67\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{red!32.1!} \makecell{10.00\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!34.1!} \makecell{7.50\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!18.7!} \makecell{25.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{red!36.5!} \makecell{10.89\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Mixtral \cite{jiang2024mixtral} & 8x7B & \cellcolor{green!10.2!} \makecell{22.63\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!11.3!} \makecell{40.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!15.0!} \makecell{6.67\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!13.6!} \makecell{17.50\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{red!26.8!} \makecell{11.25\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!40.9!} \makecell{21.25\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \cellcolor{red!41.2!} \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \cellcolor{green!2.8!} \makecell{22.35\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 8B & \cellcolor{red!6.3!} \makecell{16.51\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!18.7!} \makecell{25.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!60.0!} \makecell{1.67\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!30.0!} \makecell{7.50\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!30.4!} \makecell{10.42\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!0.0!} \makecell{13.75\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!15.0!} \makecell{26.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{red!17.6!} \makecell{16.24\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 70B & \cellcolor{green!35.5!} \makecell{33.94\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!55.9!} \makecell{66.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!31.3!} \makecell{25.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!20.5!} \makecell{20.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!10.0!} \makecell{20.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!13.6!} \makecell{16.25\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{green!12.5!} \makecell{36.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!36.4!} \makecell{35.91\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
GPT-3.5 \cite{ouyang2022training} & N/A & \cellcolor{green!5.5!} \makecell{20.49\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!19.8!} \makecell{45.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!6.3!} \makecell{11.67\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{green!13.6!} \makecell{17.50\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{red!14.3!} \makecell{14.17\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!20.5!} \makecell{10.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!3.7!} \makecell{31.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!6.6!} \makecell{23.88\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
GPT-4 \cite{openai2023gpt4} & N/A & \cellcolor{green!18.4!} \makecell{26.30\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!64.4!} \makecell{71.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!75.0!} \makecell{48.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!75.0!} \makecell{40.00\\\textcolor{gray}{\scriptsize$\pm$0.08}}  & \cellcolor{green!45.0!} \makecell{28.75\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!6.8!} \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!11.2!} \makecell{28.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!42.1!} \makecell{38.20\\\textcolor{gray}{\scriptsize$\pm$0.02}}  \\
        \midrule
        \multicolumn{10}{c}{\bf One-shot CoT Prompting} \\
        \midrule
PMC-LLaMA \cite{wu2024pmc} & 13B & \cellcolor{red!53.4!} \makecell{5.20\\\textcolor{gray}{\scriptsize$\pm$0.01}}  & \cellcolor{red!51.6!} \makecell{10.42\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!0.0!} \makecell{8.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!60.0!} \makecell{2.50\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!44.6!} \makecell{7.08\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!68.2!} \makecell{1.25\\\textcolor{gray}{\scriptsize$\pm$0.01}}  & \cellcolor{red!48.7!} \makecell{11.67\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!50.3!} \makecell{6.97\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
\textsc{MediTron} \cite{chen2023meditron} & 70B & \cellcolor{green!10.9!} \makecell{22.94\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!10.6!} \makecell{39.58\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!43.8!} \makecell{31.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!6.8!} \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!11.7!} \makecell{20.42\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!6.8!} \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{red!3.7!} \makecell{31.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!12.5!} \makecell{26.27\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Mistral \cite{jiang2023mistral} & 7B & \cellcolor{red!29.2!} \makecell{11.01\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!6.6!} \makecell{30.42\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!15.0!} \makecell{6.67\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!75.0!} \makecell{0.00\\\textcolor{gray}{\scriptsize$\pm$0.00}}  & \cellcolor{green!5.0!} \makecell{18.75\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!40.9!} \makecell{6.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!33.7!} \makecell{18.33\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \cellcolor{red!16.2!} \makecell{16.62\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Mixtral \cite{jiang2024mixtral} & 8x7B & \cellcolor{green!22.5!} \makecell{28.13\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!29.7!} \makecell{50.83\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!0.0!} \makecell{8.33\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{green!27.3!} \makecell{22.50\\\textcolor{gray}{\scriptsize$\pm$0.07}}  & \cellcolor{green!13.3!} \makecell{20.83\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!27.3!} \makecell{8.75\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!0.0!} \makecell{33.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!19.6!} \makecell{29.13\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 8B & \cellcolor{green!37.5!} \makecell{34.86\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!3.5!} \makecell{35.42\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!45.0!} \makecell{3.33\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{red!60.0!} \makecell{2.50\\\textcolor{gray}{\scriptsize$\pm$0.02}}  & \cellcolor{green!13.3!} \makecell{20.83\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{red!13.6!} \makecell{11.25\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{green!31.3!} \makecell{41.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!15.1!} \makecell{27.32\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
Llama 3 \cite{touvron2023llama2} & 70B & \cellcolor{green!52.5!} \makecell{41.59\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!38.9!} \makecell{56.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!40.6!} \makecell{30.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!27.3!} \makecell{22.50\\\textcolor{gray}{\scriptsize$\pm$0.07}}  & \cellcolor{green!48.3!} \makecell{29.58\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!75.0!} \makecell{27.50\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \cellcolor{green!43.8!} \makecell{45.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!46.4!} \makecell{39.92\\\textcolor{gray}{\scriptsize$\pm$0.02}}  \\
GPT-3.5 \cite{ouyang2022training} & N/A & \cellcolor{green!28.6!} \makecell{30.89\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!43.9!} \makecell{59.17\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!62.5!} \makecell{41.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!6.8!} \makecell{15.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!30.0!} \makecell{25.00\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!20.5!} \makecell{17.50\\\textcolor{gray}{\scriptsize$\pm$0.04}}  & \cellcolor{green!6.3!} \makecell{35.00\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!34.8!} \makecell{35.24\\\textcolor{gray}{\scriptsize$\pm$0.01}}  \\
GPT-4 \cite{openai2023gpt4} & N/A & \cellcolor{green!75.0!} \makecell{51.68\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!75.0!} \makecell{77.50\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!71.9!} \makecell{46.67\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!68.2!} \makecell{37.50\\\textcolor{gray}{\scriptsize$\pm$0.08}}  & \cellcolor{green!75.0!} \makecell{36.25\\\textcolor{gray}{\scriptsize$\pm$0.03}}  & \cellcolor{green!75.0!} \makecell{27.50\\\textcolor{gray}{\scriptsize$\pm$0.05}}  & \cellcolor{green!75.0!} \makecell{53.33\\\textcolor{gray}{\scriptsize$\pm$0.06}}  & \cellcolor{green!75.0!} \makecell{51.48\\\textcolor{gray}{\scriptsize$\pm$0.02}}  \\
        \bottomrule
    \end{tabular}
    \label{tab:main_results}
\end{table}

